A Comparison of Modern General-Purpose Visual SLAM Approaches

Advancing maturity in mobile and legged robotics technologies is changing the landscapes where robots are being deployed and found. This innovation calls for a transformation in simultaneous localization and mapping (SLAM) systems to support this new generation of service and consumer robots. No longer can traditionally robust 2D lidar systems dominate while robots are being deployed in multi-story indoor, outdoor unstructured, and urban domains with increasingly inexpensive stereo and RGB-D cameras. Visual SLAM (VSLAM) systems have been a topic of study for decades and a small number of openly available implementations have stood out: ORB-SLAM3, OpenVSLAM and RTABMap. This paper presents a comparison of these 3 modern, feature rich, and uniquely robust VSLAM techniques that have yet to be benchmarked against each other, using several different datasets spanning multiple domains negotiated by service robots. ORB-SLAM3 and OpenVSLAM each were not compared against at least one of these datasets previously in literature and we provide insight through this lens. This analysis is motivated to find general purpose, feature complete, and multi-domain VSLAM options to support a broad class of robot applications for integration into the new and improved ROS 2 Nav2 System as suitable alternatives to traditional 2D lidar solutions.

==> rebuttal.tex <==

We thank the reviewers and editors for reviewing the manuscript. All comments were addressed in the changes to the manuscript except for those described below. If any additional changes on these points should be required, we are happy to make those changes with your request. Refinements to the IMU discussion and experiments were made corresponding to all reviewer comments.

While OpenVSLAM was indeed removed from GitHub by the original authors at https://github.com/xdspacelab/openvslam due to concerns around licensing, a review of these concerns were made and deemed to be largely overblown. The broader robotics community forked this and created their own "community fork" of OpenVSLAM at https://github.com/OpenVSLAM-Community which was used for evaluation and continues to receive updates. This point was better clarified. 

Reviewer 4 suggested a new metric for estimating the proportion of failed trajectory that was successfully tracked. While we also agree this is potentially an insightful metric, we leave this for later work to analyze and is not in the direct scope intent of this paper. As this focuses on practical service robot deployments, it is less useful to analyze greatly "how much" it did before failing. The failure itself makes that technique not as suitable for practical use, as we discuss in our analysis section. 

Reviewer 4 also suggested including color maps. While this would be visually appealing, we lack the room in the paper and we do not feel there is a sufficient amount of discussion around this figure that would be worth removing more detailed and meaningful analysis from the paper to make room for it. 

Reviewer 4 also asked why not all sequences of TUM RGB-D were not used. This was explicitly called out in the paper, "... However, for service robots, the most interesting sequences are those of the "Pioneer" robot SLAM sessions." We believe that is clear and perhaps the reviewer missed it. 
